The category of opetopes and the category of opetopic sets

We give an explicit construction of the category Opetope of opetopes. We prove that the category of opetopic sets is equivalent to the category of presheaves over Opetope.

==> pic75.tex <==
% Drawing generated by LaTeX-CAD 1.9 - requires latexcad.sty 
% (c) 1998 John Leis leis@usq.edu.au 
\begin{picture}(42,34)
\thinlines
\drawcenteredtext{20.0}{28.0}{$t$}
\drawcenteredtext{8.0}{18.0}{$t'$}
\drawcenteredtext{32.0}{18.0}{$t''$}
\drawcenteredtext{20.0}{6.0}{$t'''$}
\drawdashline{10.0}{16.0}{18.0}{8.0}
\drawdashline{30.0}{16.0}{22.0}{8.0}
\drawvector{16.0}{10.0}{2.0}{1}{-1}
\drawvector{18.0}{26.0}{8.0}{-3}{-2}
\drawvector{22.0}{26.0}{8.0}{3}{-2}
\drawvector{24.0}{10.0}{2.0}{-1}{-1}
\end{picture}


==> pic76.tex <==
% Drawing generated by LaTeX-CAD 1.9 - requires latexcad.sty 
% (c) 1998 John Leis leis@usq.edu.au 
\begin{picture}(40,22)
\thinlines
\drawcenteredtext{18.0}{16.0}{$t$}
\drawcenteredtext{8.0}{6.0}{$t'$}
\drawcenteredtext{30.0}{6.0}{$t''$}
\drawvector{16.0}{14.0}{8.0}{-3}{-2}
\drawvector{20.0}{14.0}{8.0}{3}{-2}
\end{picture}

